Brain-inspired Search Engine Assistant based on Knowledge Graph

Search engines can quickly response a hyperlink list according to query keywords. However, when a query is complex, developers need to repeatedly refine the search keywords and open a large number of web pages to find and summarize answers. Many research works of question and answering (Q and A) system attempt to assist search engines by providing simple, accurate and understandable answers. However, without original semantic contexts, these answers lack explainability, making them difficult for users to trust and adopt. In this paper, a brain-inspired search engine assistant named DeveloperBot based on knowledge graph is proposed, which aligns to the cognitive process of human and has the capacity to answer complex queries with explainability. Specifically, DeveloperBot firstly constructs a multi-layer query graph by splitting a complex multi-constraint query into several ordered constraints. Then it models the constraint reasoning process as subgraph search process inspired by the spreading activation model of cognitive science. In the end, novel features of the subgraph will be extracted for decision-making. The corresponding reasoning subgraph and answer confidence will be derived as explanations. The results of the decision-making demonstrate that DeveloperBot can estimate the answers and answer confidences with high accuracy. We implement a prototype and conduct a user study to evaluate whether and how the direct answers and the explanations provided by DeveloperBot can assist developers' information needs.

==> botLearning.tex <==
\subsection{\emph{BotLearning}: Knowledge Graph of Software Engineering Domain Construction}\label{botMemory}
%\subsubsection{Knowledge Graph Construction}
The backend knowledge base of the \emph{DeveloperBot} is a knowledge graph of software engineering domain which combines the advance domain knowledge graph extract techniques~\cite{zhao2017hdskg,li2018improving,zhaohdso} and the expertise of domain experts.
In this section, we summarize the key points of these techniques.
Refer to our paper for more technical details~\cite{zhao2017hdskg,li2018improving,zhaohdso}.

\subsubsection{The Data Source -- Tag Wiki of Stack Overflow}
When ask questions on Stack Overflow, the users will be asked to put 1-5 tags as a short description of this question so that the Stack Overflow can easy to classify the questions.
Tag is technical term~(e.g. windows, graph database, javascript, etc.) involving a wide range of content from operating system, programming languages, libraries, to specific APIs~\cite{chen2016techland}.
%The tag wiki is a general introduction and definition of a tag as shown in Fig.~\ref{tagwikiFirebird}.
The tag wiki is a general introduction and definition of a tag.
%\begin{figure*}[htb]
%    \centering
%    \includegraphics[width=3.7in]{developerBot/tagwikiFirebird.pdf}
%    \caption {Tag Wiki of Tag ``firebird''}
%    \label{tagwikiFirebird}
%\end{figure*}

Stack Overflow is strict to create new tag~\footnote[1]{http://stackoverflow.com/help/privileges/create-tags} and edit the tag wiki~\footnote[2]{https://stackoverflow.com/help/privileges/approve-tag-wiki-edits}.
The community also pays a lot of effort to maintain and organize the tag wikis.
As a result, the tag wikis of Stack Overflow tags have the advantages of accurate tag introduction, comprehensive technical coverage and standard grammatical structure for constructing the knowledge graph of software engineering domain.

\subsubsection{Domain Knowledge Graph Construction}
Type information of knowledge graph (KG) entities is an important feature that
categorizes entities of similar semantics. It is used in different tasks related to
knowledge graphs including meta path extraction [1], link prediction [2] and fact
checking [3]. Naturally, knowledge entities are categorized into a hierarchically
structured set of classes e.g., person ) artist ) singer, or location ) country
) city, where each class encloses entities of similar properties. Hierarchical
class structure provides richer semantics of entity type information that can
be used as a feature in different knowledge graph tasks e.g. link prediction
and entity linking [4]. Despite their usefulness, famous knowledge graphs from
different domains suffer from type assertion incompleteness [5].

\subsubsection{Augment Knowledge Graph by Expertise of Domain Experts}
In addition to the advantages of the tag wiki mentioned above, it also has its limitations.
For example, there are some relations that are very important in the software engineering domain, but they are rarely mentioned in natural language because these relations are too common sense~(e.g. ``A graph database is a database.'').

Crowdsourcing data is edited by different user, so there are often different expressions for the relation.
For example, a relation (doxygen, is\_available\_for, Linux) is same mean as (doxygen, run\_on, Linux).
There are also some different expressions point to the same concept like ``object-database'' and ``object-oriented-database'' are the same meaning.
Stack Overflow provides a synonym set~\footnote[1]{https://stackoverflow.com/tags/synonyms} with more that 4000 synonyms in software engineering domain.
These synonyms is incorporated into the domain knowledge graph with relation ``is\_synonym\_of''~(e.g. mpmjs; is\_synonym\_of; npm) for further analysis.
%There are some common relations with multiple representations in software engineering domain.

There are also some equivalence relations in the software engineering domain.
For example, if there is a relation (P4V; is; cross\_platform)~\footnote[2]{https://stackoverflow.com/tags/p4v/info}.
A cross-platform application may run on Microsoft Windows, Linux, and macOS ~\footnote[3]{https://en.wikipedia.org/wiki/Cross-platform\_software}.
So we can derive relations that (P4V; run\_on; Microsoft\_Windows), (P4V; run\_on; Linux) and (P4V; run\_on; macOS)~\footnote[4]{https://www.perforce.com/downloads/helix-visual-client-p4v}.
%('23910_0_0', 'SWFUpload', 'is', 'JavaScript/Flash_library')
%('23910_0_0', 'SWFUpload', 'is', 'Flash_library')
%\subsubsection{Structural Data Augmentation}
%A the leaf of example of query "database written in microsoft language"
%['relational database', 'knowledge base', 'object relational database', 'xml database', 'object database', 'document oriented database', 'graph database', 'mysql', 'sqlite', 'oracle database', 'foxpro', 'data warehouse', 'microsoft sql server', 'advantage database server', 'sql anywhere', 'dataflex', 'hsqldb', 'firebird', 'oracle database', 'exasolution', 'wikidata', 'postgresql', 'exist db', 'perst', 'objectivity db', 'wikidata', 'mongodb', 'neo4j', 'titan', 'bitsy', 'cayley', 'arangodb', 'titan']
%['c++', 'c#', 'c', 'visual basic', 'jscript', 'php', 'ironpython', 'ironruby']
%JS library to javascript library
%unix operating system to unix
% relational database management system
%suse to SUSE linux

\subsubsection{Augment Knowledge Graph by NLP Techniques}
In addition, there are also some implicit relations between some entities, which can be identified by syntax.
The ``head''~\footnote[5]{https://en.wikipedia.org/wiki/Head\_(linguistics)} of a phrase is the word that determines the syntactic category of that phrase.
For example, ``red dog'' is a ``dog'', the word ``red'' of the phrase modify the head, and is therefore the head's dependents.
Here we extend the syntax rule ``head'' to the entity level.
Assume there are two entities in the knowledge graph named entity$_1$ and entity$_2$, if entity$_1$ is the head of entity$_2$, a hierarchical relation (entity$_2$; is\_a; entity$_1$) will be built in the knowledge graph.
For example, if entity$_1$ is ``programming\_language'' and entity$_2$ is ``object-oriented\_programming\_language''.
The entity ``programming\_language'' is the head of ``object-oriented\_programming\_language'' since the ``object-oriented'' modify this head entity ``programming\_language'', so ``object-oriented'' is  dependent of ``programming\_language''.
So we can derive a relation that (object-oriented\_programming\_language; is\_a; programming\_language)

%Type information of knowledge graph (KG) entities is an important feature that categorizes entities of similar semantics. It is used in different tasks related to knowledge graphs including meta path extraction , link predictionand fact checking .Naturally, knowledge entities are categorized into a hierarchically structured set of classes e.g. , person artist  singer, or location country city, where each class encloses entities of similar properties. Hierarchical class structure provides richer semantics of entity type information that can be used as a feature in different knowledge graph tasks e.g. link prediction and entity linking [ 4]. D

Named-entity recognition (NER) (also known as entity identification, entity chunking and entity extraction) seeks to locate and classify sequences of words in a text into pre-defined categories such as person and company names, or gene and protein names, organizations, locations, medical codes, time expressions, etc.
The \emph{DeveloperBot} incorporates the tool named \emph{coreNLP} released by Stanford to recognize all the entities in the final knowledge graph~\cite{manning2014stanford,toutanova2000enriching,nivre2016universal,schuster2016enhanced}.
%\begin{figure}[hbt]
%    \centering
%    \includegraphics[width=3in]{developerBot/NER_example.pdf}
%    \caption {Result of Named-entity Recognition for Relation Triple (Microsoft, was\_founded\_by, Bill\_Gates)}
%    \label{ner}
%\end{figure}
%As shown in Fig.~\ref{ner}, 
The relation triple (Microsoft, was\_founded\_by, Bill\_Gates) is recognized two named-entities, they are ``Microsoft''-ORGANIZATION and ``Bill Gates''-PERSON.
So two relation triples (Microsoft, is\_a, organization) and (Bill\_Gates, is\_a, person) will be added into the knowledge graph.


==> botMemory.tex <==
\subsection{\emph{BotMemory}: Knowledge Graph of Software Engineering Domain Construction}\label{botMemory}
%\subsubsection{Knowledge Graph Construction}
The backend knowledge base of the \emph{DeveloperBot} is a knowledge graph of software engineering domain which combines the advance domain knowledge graph extract techniques~\cite{zhao2017hdskg,li2018improving,zhaohdso} and the expertise of domain experts.
In this section, we summarize the key points of these techniques.
Refer to our paper for more technical details~\cite{zhao2017hdskg,li2018improving,zhaohdso}.

\subsubsection{The Data Source -- Tag Wiki of Stack Overflow}
When ask questions on Stack Overflow, the users will be asked to put 1-5 tags as a short description of this question so that the Stack Overflow can easy to classify the questions.
Tag is technical term~(e.g. windows, graph database, javascript, etc.) involving a wide range of content from operating system, programming languages, libraries, to specific APIs~\cite{chen2016techland}.
The tag wiki is a general introduction and definition of a tag as shown in Fig.~\ref{tagwikiFirebird}.
Stack Overflow is strict to create new tag~\footnote[1]{http://stackoverflow.com/help/privileges/create-tags} and edit the tag wiki~\footnote[2]{https://stackoverflow.com/help/privileges/approve-tag-wiki-edits}.
The community also pays a lot of effort to maintain and organize the tag wikis.
As a result, the tag wikis of Stack Overflow tags have the advantages of accurate tag introduction, comprehensive technical coverage and standard grammatical structure for constructing the knowledge graph of software engineering domain.
\begin{figure}
    \centering
    \includegraphics[width=3in]{developerBot/tagwikiFirebird.pdf}
    \caption {Tag Wiki of Tag ``firebird''}
    \label{tagwikiFirebird}
\end{figure}

\subsubsection{Domain Knowledge Graph Construction}
Type information of knowledge graph (KG) entities is an important feature that
categorizes entities of similar semantics. It is used in different tasks related to
knowledge graphs including meta path extraction [1], link prediction [2] and fact
checking [3]. Naturally, knowledge entities are categorized into a hierarchically
structured set of classes e.g., person ) artist ) singer, or location ) country
) city, where each class encloses entities of similar properties. Hierarchical
class structure provides richer semantics of entity type information that can
be used as a feature in different knowledge graph tasks e.g. link prediction
and entity linking [4]. Despite their usefulness, famous knowledge graphs from
different domains suffer from type assertion incompleteness [5].

\subsubsection{Augment Knowledge Graph by Expertise of Domain Experts}
In addition to the advantages of the tag wiki mentioned above, it also has its limitations.
For example, there are some relations that are very important in the software engineering domain, but they are rarely mentioned in natural language because these relations are too common sense~(e.g. ``A graph database is a database.'').

Crowdsourcing data is edited by different user, so there are often different expressions for the relation.
For example, a relation (doxygen, is\_available\_for, Linux) is same mean as (doxygen, run\_on, Linux).
There are also some different expressions point to the same concept like ``object-database'' and ``object-oriented-database'' are the same meaning.
Stack Overflow provides a synonym set~\footnote[1]{https://stackoverflow.com/tags/synonyms} with more that 4000 synonyms in software engineering domain.
These synonyms is incorporated into the domain knowledge graph with relation ``is\_synonym\_of''~(e.g. mpmjs; is\_synonym\_of; npm) for further analysis.
%There are some common relations with multiple representations in software engineering domain.

There are also some equivalence relations in the software engineering domain.
For example, if there is a relation (P4V; is; cross\_platform)~\footnote[1]{https://stackoverflow.com/tags/p4v/info}.
A cross-platform application may run on Microsoft Windows, Linux, and macOS ~\footnote[1]{https://en.wikipedia.org/wiki/Cross-platform\_software}.
So we can derive relations that (P4V; run\_on; Microsoft\_Windows), (P4V; run\_on; Linux) and (P4V; run\_on; macOS)~\footnote[1]{https://www.perforce.com/downloads/helix-visual-client-p4v}.
%('23910_0_0', 'SWFUpload', 'is', 'JavaScript/Flash_library')
%('23910_0_0', 'SWFUpload', 'is', 'Flash_library')
%\subsubsection{Structural Data Augmentation}
%A the leaf of example of query "database written in microsoft language"
%['relational database', 'knowledge base', 'object relational database', 'xml database', 'object database', 'document oriented database', 'graph database', 'mysql', 'sqlite', 'oracle database', 'foxpro', 'data warehouse', 'microsoft sql server', 'advantage database server', 'sql anywhere', 'dataflex', 'hsqldb', 'firebird', 'oracle database', 'exasolution', 'wikidata', 'postgresql', 'exist db', 'perst', 'objectivity db', 'wikidata', 'mongodb', 'neo4j', 'titan', 'bitsy', 'cayley', 'arangodb', 'titan']
%['c++', 'c#', 'c', 'visual basic', 'jscript', 'php', 'ironpython', 'ironruby']
%JS library to javascript library
%unix operating system to unix
% relational database management system
%suse to SUSE linux

\subsubsection{Augment Knowledge Graph by NLP Techniques}
In addition, there are also some implicit relations between some entities, which can be identified by syntax.
The ``head''~\footnote[1]{https://en.wikipedia.org/wiki/Head\_(linguistics)} of a phrase is the word that determines the syntactic category of that phrase.
For example, ``red dog'' is a ``dog'', the word ``red'' of the phrase modify the head, and is therefore the head's dependents.
Here we extend the syntax rule ``head'' to the entity level.
Assume there are two entities in the knowledge graph named entity$_1$ and entity$_2$, if entity$_1$ is the head of entity$_2$, a hierarchical relation (entity$_2$; is\_a; entity$_1$) will be built in the knowledge graph.
For example, if entity$_1$ is ``programming\_language'' and entity$_2$ is ``object-oriented\_programming\_language''.
The entity ``programming\_language'' is the head of ``object-oriented\_programming\_language'' since the ``object-oriented'' modify this head entity ``programming\_language'', so ``object-oriented'' is  dependent of ``programming\_language''.
So we can derive a relation that (object-oriented\_programming\_language; is\_a; programming\_language)

%Type information of knowledge graph (KG) entities is an important feature that categorizes entities of similar semantics. It is used in different tasks related to knowledge graphs including meta path extraction , link predictionand fact checking .Naturally, knowledge entities are categorized into a hierarchically structured set of classes e.g. , person artist  singer, or location country city, where each class encloses entities of similar properties. Hierarchical class structure provides richer semantics of entity type information that can be used as a feature in different knowledge graph tasks e.g. link prediction and entity linking [ 4]. D

Named-entity recognition (NER) (also known as entity identification, entity chunking and entity extraction) seeks to locate and classify sequences of words in a text into pre-defined categories such as person and company names, or gene and protein names, organizations, locations, medical codes, time expressions, etc.
The \emph{DeveloperBot} incorporates the tool named \emph{coreNLP} released by Stanford to recognize all the entities in the final knowledge. graph~\cite{manning2014stanford,toutanova2000enriching,nivre2016universal,schuster2016enhanced}.

\begin{figure}
    \centering
    \includegraphics[width=2.5in]{developerBot/NER_example.pdf}
    \caption {Result of Named-entity Recognition for Relation Triple (Microsoft, was\_founded\_by, Bill\_Gates)}
    \label{ner}
\end{figure}

As shown in Fig.~\ref{ner}, the relation triple (Microsoft, was\_founded\_by, Bill\_Gates) is recognized two named-entities, they are ``Microsoft''-ORGANIZATION and ``Bill Gates''-PERSON.
So two relation triples (Microsoft, is\_a, organization) and (Bill\_Gates, is\_a, person) will be added into the knowledge graph.


==> introduction.tex <==
\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%
% Search engine is important and dominant for developer's information need.
%%%%%%%%%%%%%%%%%%%%%
Many studies and our preliminary survey show that web search engines are the most dominant, prominent and indispensable tool for developers to search online information resources or solve problems currently~\cite{singer2013ordinary,cho2004impact,zhao2018smart,li2015amassist}.
Today's web search engines are primarily follows the ``query-response'' or short lookup concept.
The developers use these web search engines for a variety of search tasks by type queries and receive ranked lists of search results~(or say hyperlinks)~\cite{singer2013ordinary}.
%--- from simple lookups to complex information needs ---
%Some studies show that the traditional document ranking and linked data based web search engines support the simple search tasks very well and satisfying for the users~\cite{lewandowski2008retrieval,singer2013ordinary}.the community of IR~(Information Retrieval)

%%%%%%%%%%%%%%%%%%%%%
% The shortcoming of current search engine technologies: good at handle simple query, but weak in handle complex information needs, example of a queries to Google.
%%%%%%%%%%%%%%%%%%%%%
Recently, the community of search engine users is increasingly recognizing that traditional retrieval models are insufficient to satisfy complex information needs~\cite{sarrafzadeh2014exploring,carlson2003information,singer2013ordinary}.
For example, if a developer type the following query in a search engine - ``data visualization library for javascript''.
The received list of search results is reasonable since developers only need to click on a few hyperlinks to get the information they want.
But try this query - ``Which graph databases is compatible with Linux and supports both Java and Python?''.
The list of returned results is far from satisfactory.
In order to get the information they want, the developer have to open a lot of hyperlinks and synthesize the results of different sources related to their information needs~\cite{singer2013ordinary}.
The above two queries are very easy to understand for humans, but current NLP-based web search engines still can't perform well on complex queries ~\cite{zhu2015building}.
%an increasing number of users use search engines to aggregate information to support their decisions making~\cite{weitz2009search}.
%The point of this system is that it simplifies searching. Many times when we use a search engine, were just looking for something really simple or trivial. Returning a long list of results doesnt seem like the most efficient way of answering the question, even though the answer is almost certainly hidden away in those results.

%%%%%%%%%%%%%%%%%%%%%
% Developers have huge need for complex information search, and how developers current do for these need, and what the weak point for these solutions.
%%%%%%%%%%%%%%%%%%%%%
Nowadays, developers have many alternative solutions for complex information needs.
The Q\&A websites like Quora and Stack Overflow that allow developers to post complex questions are popular search engine supplements.
According to our rough statistics, 23\% of the questions on Stack Overflow are closed-ended questions, which means the questions are used to obtain facts or specific direct answer~\footnote[1]{Here we counted the questions on Stack Overflow that the first letter is ``which'' or ``what'' and followed by a noun phrase.}.
%~(e.g. \href{https://stackoverflow.com/questions/9703121/which-database-to-use-with-django}{Question:Which database to use with Django? Answer:SQLite, MySQL, PostgreSQL})~\cite{closedEndedQuestion}).
So obviously, developers have a huge need for complex information search that provide specific direct answers

%but whether they synthesize the results of search engines or ask questions on the Q\&A websites, it takes a lot of time and effort to get the answer they want.

%When the developers fail to search for the information resources,
%~(e.g. \href{https://www.quora.com/Which-Linux-Distros-support-Oracle-Database-installations}{Which Linux Distros support Oracle Database installations?})
%before they star to programming~
%or when their programming stop by error~(e.g. \href{https://community.oracle.com/thread/4265917}{Oracle 19c for Linux Debian})
%(e.g. \href{https://stackoverflow.com/questions/9703121/which-database-to-use-with-django}{Which database to use with Django?})

%%%%%%%%%%%%%%%%%%%%%
% How question answer system work and why it important to solve the above issues, what the attitude to the question answer system of the industry like Google. Why explainability is important.
%%%%%%%%%%%%%%%%%%%%%
%Based on the above situation, in order to provide web search engine users with better support on complex search tasks, many researches proposal provide additional enhanced services for complex search tasks depending on their characters~\cite{singer2013ordinary}.
%This is a consensus for major search engine companies (e.g. Google, Bing, Yahoo, etc.): automatic Question Answering (QA) system~(also known as direct answer search engine, or natural language search engine, etc.) is a more advanced next-generation search engine which return real-time answers instead of a ranked list of hyperlinks~\cite{Google,Google2,Bing,Yahoo}.
%But it is one of the more difficult tasks in the field of natural language processing (NLP) because it requires a wide range of intelligence (parsing, search, information extraction, coreference, inference).

%%%%%%%%%%%%%%%%%%%%%
% What algorithm include and what our tool include and what our tool can do.
%%%%%%%%%%%%%%%%%%%%%
In this paper, we explore the content of cognitive science related to complex problem perception, planning, and reasoning based on semantic memory~\cite{giguere2013limits,matlin1992sensation,owen1997cognitive,collins1975spreading}.
Although the cognitive process of the human brain for these kinds of advanced tasks is complex and the cognitive scientists do not yet reach a final consensus~\cite{lisman2015challenge}.
But some of the research achievements have made it possible to connect a complex question solving to cognitive process.
We propose a brain-inspired framework named \emph{DeveloperBot} which is consistent with cognitive process of human and have the capacity to answer complex queries with explainability based on a knowledge graph.
Just like humans, what kind of questions \emph{DeveloperBot} can answer depends on what knowledge it has learned.
Even when some questions exceed the knowledge it has, \emph{DeveloperBot} can also provide reasoning answers, explanations and confidence values based on the mastered knowledge.

\emph{DeveloperBot} consists of four main modules, (1) \emph{BotPerception}: constructs query graph, (2) \emph{BotPlanning}: divides a query into smaller queries and decides the right solving order, (3) \emph{BotReasoning}: searches the knowledge graph, makes the decisions, reasons final answers, extracts the explanation and computes the confidence, (4) \emph{BotReponse} presents the answers by UI~(user interface).
\emph{BotPerception} and \emph{BotPlanning} incorporates the Dependency Parsing into the Tree Parsing~\cite{fellbaum1998semantic} for maximizing the extraction of answers constraints to a query graph, and then planing the solving order of these constraints.
\emph{BotReasoning} inspires from spreading activation model~\cite{collins1975spreading} and combines logic rules and data to model the question solving as subgraph search and Bayesian decision making process.

%Then we use the extracted query target and its constraint description to perform a fast traversal algorithm to the knowledge graph.
%If we find the direct answers that meet the requirements, we will return a list of direct answers and their confidence, path of knowledge graph path for direct answer reasoning as the explanation of the direct answers, similar objects of the query target, and the briefs and relation graphs of the entities in the query.
%Since the fast traversal algorithm is based on text matching, it can obtain high-accuracy matching results quickly.
%If the fast traversal algorithm fail to find an answer, we will perform a topology matching and path ranking algorithm then return the top 10 answers with confidence and their reasoning path as an explanation so that the user can further determine if the answer is what they want.

%With the knowledge graph of software engineering domain and query graph, we propose an algorithm that can search the direct answers of the multi-constrained query graph from the domain knowledge graph, called fast knowledge graph cyclic pruning algorithm~(\emph{BotBrain-Logic}).
%Furthermore, \emph{BotBrain-Logic} can also construct a subgraph of the inference path of the direct answer and calculate the confidence of the direct answer.
%The subgraph and the confidence can be used as an explanation for the direct answer, providing decision support for the developers.
%The recommended similar entities and Structured Wiki can assist the developers to do exploratory search, which allows the developers to understand their queries more deeply, in order to form better query keywords to make their information needs description more accurate.

%\emph{DeveloperBot} has functions of complex query
%understanding and inference, explainable direct answer searching, confidence of direct answer computation, similar entities recommendation and query interpretation~(called Structured Wiki in our work), etc.
%In order to achieve the above functions, we use our previous tool \emph{HDSKG}~\cite{zhao2017hdskg} to exploit the crowdsourcing knowledge of Stack Overflow to construct a knowledge graph of software engineering domain.
%\emph{HDSKG} can extract basic elements of the knowledge graph -- relation triples like (subject, verb phrase, object) -- from the natural language text materials automatically, and estimate the domain relevance to exclude relational triples that are not belong to the specified domain.
%Then some domain experts further assist in the correction, supplementation, refinement and completion of the knowledge graph.

We implement a prototype of \emph{DeveloperBot} for evaluation and train it by the knowledge graph of software engineering domain.
Then we use it as a search engine assistant specific for developers.
First, we collect a repository including 100 questions and their corresponding answers from developers.
90 of these questions are used to evaluate the accuracy of \emph{DeveloperBot} compared with the popular search engines~(e.g. Google, WolframAlpha, etc.).
Then a user study involving 20 developers is conducted with the rest 10 question.
The results show that \emph{DeveloperBot} has capacity to model and reason complex problems with high accuracy.
And compared with the developers who use search engine~(e.g. Google) only, the developers who use both \emph{DeveloperBot} and search engine can get the answers they want faster and more efficient.
In addition, the explanations and confidences of answers can assist developers to understand the answers furtherly, filter the unwanted answers and improve the developers' trust to the answers.
%
%The results indicate that \emph{DeveloperBot} can answer most of the closed-ended questions on Stack Overflow with high-accuracy and \emph{DeveloperBot} also exhibits greater flexibility in answering a variety of questions.

%The explanations and confidence we provide can help users to better correct the wrong answers and find the information they want effectively.
%And the recommended similar entities and Structured Wiki can assist the developers to form better query keywords effectively.



%%%%%%%%%%%%%%%%%%%%%
% The prototype and evaluation.
%%%%%%%%%%%%%%%%%%%%%
%We build a prototype of the \emph{DeveloperBot}~(including both the backend searching algorithm and the frontend web-based application) and release the system for the community of developers to use.
%Before release, we evaluate the usefulness and effectiveness of the \emph{DeveloperBot} in assisting complex information needs by an experiment and an user study respectively.
%Specifically, we first use \emph{DeveloperBot} to query 100 closed-ended questions on Stack Overflow, and analyze the result.
%Second, we evaluate the usability and the acceptability of \emph{DeveloperBot} by 20 participants.
%It is important to note that our knowledge graph is extract from the Tagwiki of Stack Overflow and involves more than ?? popular programming language and their library, framework, API, etc. Thus it presents an high-accuracy, broad coverage and strong timeliness.

%%%%%%%%%%%%%%%%%%%%%
% Summarize the contribution of our paper
%%%%%%%%%%%%%%%%%%%%%
This paper makes following four major contributions:
\begin{itemize}
  \item [1)] A brain-inspired framework named \emph{DeveloperBot} is proposed, which is consistent with cognitive process of human and have the capacity to answer complex queries with explainability based on knowledge graph.
  \item [2)] We propose the emph{BotPerception} and \emph{BotPlanning} algorithms which incorporate the Dependency Parsing into the Tree Parsing to divide a complex query into smaller queries and decides the right solving order, then construct these into a query graph.    
  \item [3)] A algorithm named \emph{BotReasoning} is proposed, which inspires from spreading activation model and models the question solving as subgraph search and Bayesian decision making process.
      \emph{BotReasoning} also extracts the reasoning subgraph and computes the confidence values as qualitative and quantitative explanations to the corresponding direct answers respectively.
  \item [4)] The prototype of \emph{DeveloperBot} system is implemented and trained by a knowledge graph of software engineering domain for accuracy and efficiency evaluation.
  
  % quality of \emph{DeveloperBot} is evaluated by either employing a set of quantitative and qualitative methods including analyzing the accuracy of direct answers by 100 closed-ended questions on Stack Overflow and a user study directly reflecting the effectiveness, usefulness and acceptability.
  % We analyze the results of the automatic knowledge graph extraction tool \emph{HDSKG}, and propose an knowledge graph enhancement scheme, and finally publish a knowledge graph of software engineering domain with 44800 concepts, 9660 unique verb phrase and 35279 relation triples~\footnote[1]{http://neo4j.tuntunkun.org/xuejiao/}.
  % \item [3)] We propose an fast knowledge graph cyclic pruning algorithm called \emph{BotBrain-Logic} that can search the direct answers of the multi-constrained query graph from the domain knowledge graph.
  % \emph{BotBrain-Logic} can also construct a subgraph of the derived paths of the direct answer and calculate the confidence of the direct answer as qualitative and quantitative explanations of the direct answer respectively.
  %  \item [2)] A multi-constrained query graph construction algorithm is proposed, which incorporates the Dependency Parsing with Tree Parsing for maximizing the extraction of constraints describing the answers of the complex query, and then construct these constraints into a query graph.
  % two empirical studies are conducted to evaluate the accuracy, effectiveness, usefulness and acceptability of \emph{DeveloperBot}.
  %\item We present a fast traversal algorithm that traverses the knowledge graph to match answers quickly based on search targets and its constraints.
  %\item we propose an method combining topological matching and path ranking algorithm. The method first searches for subgraphs that meet the topological structure of query target constraints, then uses advanced WordEmbedding algorithm to rank the paths of subgraph and responds the speculative answers and its confidence.
  %\item We implement and release the \emph{DeveloperBot} system prototype for the community of developers to use.
  %\item The prototype of \emph{DeveloperBot} system is implemented and report our field deployment and two empirical studies to evaluate the accuracy, effectiveness, usefulness and acceptability of \emph{DeveloperBot} .
\end{itemize}


%Artificial intelligence evolves with the development of computers even rely on computational development.
% The ways and processes of human thinking developed by Psychologists and welcomed by computational experts produce the science of Artificial Intelligence.
% This continues with the development of cognitive science that encourages the development of Artificial Intelligence to Cognitive Thinking Intelligence, a new pathway to the science of Artificial Intelligence that can emulate human cognitive abilities even if not 100\%.
%
%
% Emulation of human cognitive abilities is developed based on the modeling of system interaction with the environment and information fusion, which can be used to conduct Inferencing, so when this occurs repeatedly it will produce knowledge that grows. This process is called Knowledge Growing System which is Brain Inspired Cognitive Artificial Intelligence and can be used for information extraction and when applied to instrumentation system will realize Intelligent Instrumentation System.


%
%Such a system is called an automatic Question Answering (QA) system, or a Natural Language search engine. It is not to be confused with a social Question Answering service, where answers are produced by humans. QA is a well studied area, as evidenced by almost a decade of TREC QA track publications, but it is one of the more difficult tasks in the field of natural language processing (NLP) because it requires a wide range of intelligence (parsing, search, information extraction, coreference, inference). This may explain why there are relatively few freely available online systems today, most of which are more like demos. Several include:


%Google Featured Snippets  Direct Answers
%Futher more, Google engineers are constantly developing the search algorithm to make it the most consistent with mobile
%standards and voice search adapted
%improve the need of direct answer.
%
%
%
%
%Towards the goal of scaling up the large-scale, diverse and heterogeneous visual querying tasks, a handful of recent papers [7, 59] have suggested to cast the visual recognition tasks into a framework that enables more heterogeneous reasoning and inference.
%
%Mobile and voice search are shaping the future of SEO, and Google is putting new emphasis on 'direct answers' to queries. Here's what digital marketers, content creators and SEO experts need to know about these key changes.
%
%Just as important as mobile, however, is voice. Professionals who practice SEO must prepare for a future in which queries come from voice input on mobile devices, and where Google, to satisfy those voice (and text) queries, will increasingly highlight "direct answers."
%
%Google (and to a lesser extent, Bing) searches yield direct answer results, also known as "rich answers," in response to specific user questions, instead of delivering an assortment of links to other websites.
%
%In a recent evaluation of more than 850,000 search queries, Google served up some form of direct answer 19.5 percent of the time, according to Eric Enge, CEO of Stone Temple Consulting, the company that conducted the test.
%
%Especially can be use in voice search!!!
%Google is likely to respond to voice searches with direct answers, rather than links, because most voice searches are currently performed on mobile devices and mobile users want immediate answers on their small screens, Enge said. (Google comprises nearly 65 percent of the overall search market, so it's no surprise that direct answers were a hot topic at SMX West 2015.)
%
%Which can link Google also uses lists, Wikipedia entries, charts, forms, and carousels in its direct answers into the direct answer of knowledge graph.
%
%
%Some error caused by didn't search property result.
%
%
%Using Neo4j database from C++

%The complexity of the visual world creates significant challenges for comprehensive visual understanding.
%In spite of recent successes in visual recognition, todays vision systems would still struggle to deal with visual queries that require a deeper reasoning.
%The answers are far from satisfying. Both questions are perfectly clear to most humans, but current NLPbased algorithms still fail to perform well for more complex queries. In vision, we see a similar pattern.
%Much progress has been made in tasks such as classification and detection on single objects (e.g., Fig. 1(a)). But real-world vision applications might require more diverse and heterogeneous querying needs (e.g., Fig. 1(b)).
%The traditional classification-based methods would struggle in such tasks.
%A part of the problem is that we do not know enough about users searching behaviour under these circumstances.
%While many studies on user behaviour have been conducted, studies seldom differentiate explicitly between simple and complex search tasks in the sense mentioned.

%eSead can, Dash inlcule, involve many programming languages, frameworks and libraries, including: ActionScript, Android, C++, CAppuccino, Cocos2D, Cocos3D, Corona, CSS, Django, Groovy, HTML, Java, JavaFX, JavaScript, jQuery, Kobold2D, Lua, MySQL, Node.js, Man Pages, Perl, PHP, Python, Ruby, Ruby on Rails, Scala, Sparrow, SQLite, Unity 3D, WordPress, XSLT, XUL


==> introduction2_hk.tex <==
\section{Introduction}
% Current search engine good at handle easy searching, but there are many complex information needs.

% The shortcoming of current search engine technologies, including relevance driven, can't handle complex query(example of a question which google returns) .

% What the developer current do for such a information needs.
Some error caused by didn't search property result.

Post questions on Q\&A websites like Quora~(e.g. \href{https://www.quora.com/Which-Linux-Distros-support-Oracle-Database-installations}{Which Linux Distros support Oracle Database installations?}) and Stack Overflow~ before they star to programming~(e.g. \href{https://stackoverflow.com/questions/4952421/what-languages-does-django-support-i-cant-find-a-comprehensive-list}{What Languages does Django support? I can't find a comprehensive list}) or when their programming stop by error~(e.g. \href{https://community.oracle.com/thread/4265917}{Oracle 19c for Linux Debian}).

Using Neo4j database from C++


% What algorithm include and what our tool include and what our tool can do.
eSead can, Dash inlcule, involve many programming languages, frameworks and libraries, including: ActionScript, Android, C++, CAppuccino, Cocos2D, Cocos3D, Corona, CSS, Django, Groovy, HTML, Java, JavaFX, JavaScript, jQuery, Kobold2D, Lua, MySQL, Node.js, Man Pages, Perl, PHP, Python, Ruby, Ruby on Rails, Scala, Sparrow, SQLite, Unity 3D, WordPress, XSLT, XUL

% Summarize the contribution of our paper



The concept of relevance? sometimes also called pertinence?or aboutness? is central to the theory of information retrieval. Unfortunately, however,
 The purpose of this paper is to propose and defend a definition of what it means to say that a piece of stored information is relevant?to the information need of a retrieval system user.

Our knowledge graph cover xx kinds of programming language, xx unique entities and xx relations.

First, answering a variety of heterogeneous visual
queries without re-training. In real-world vision applications, the space of possible queries is huge (even infinite). It is impossible to retrain classifiers for every type
of queries. Our system demonstrates its ability to perform
reasoning and inference on an assortment of visual querying tasks, ranging from scene classification, image search to
real-world application queries, without the need to train new
classifiers for new tasks. We formalize answering these visual queries as computing the marginal probabilities of the
joint probability model (Sec. 5). The key technique is to express visual queries in a logical form that can be answered
from the visual KB in a principled inference method. We
qualitatively evaluate our KB model in answering application queries like the ones in Fig. 1 (Sec. 6.1). We then
perform quantitative evaluations on the recognition tasks
(Sec. 6.2) and retrieval tasks (Sec. 6.3) respectively using
the SUN dataset [50]. Our system achieves competitive results compared to the classification-based baseline models,
while exhibiting greater flexibility in answering a variety of
visual queries.

We then perform quantitative evaluations on the recognition tasks (Sec. 6.2) and retrieval tasks (Sec. 6.3) respectively using
the SUN dataset [50]. Our system achieves competitive results compared to the classification-based baseline models,
while exhibiting greater flexibility in answering a variety of
visual queries.

To overcome the above limitations, we propose the TechLand system that exploits the crowdsourced knowledge from
Stack Overflow, and assists technology landscape inquiries
with an informative summary of available technologies, technology correlations, and technology trend. Inspired by the
recent empirical studies on Stack Overflow [2], [1], [3],
[4], we consider question tags as technologies used by the
community, and propose association rule mining and natural
language processing methods to mine relational and categorical knowledge of technologies.


We build a prototype of the TechLand system (including the
backend knowledge base and the frontend browser plugin and
website) and release the system for public use.



The Google
Analytics of the websites 6-months visit data indicates the
general interests in our technology landscape service. We
evaluate the usefulness of the TechLand system in assisting
technology landscape inquiries in two studies. First, we evaluate the usefulness of the TechLand recommendation against the
community answers to 100 technology landscape questions on
Stack Overflow. Second, we evaluate the design and usability
of the TechLand system by a user study of 12 participants. It
is important to note that the knowledge that TechLand uses to
augment technology landscape inquiries is not based on one or
two persons?opinions. Instead, the knowledge is aggregated
from millions of questions mentioning the relevant technologies, and thus presents an objective, consistent and organized
summary for addressing the information needs in technology
landscape inquiries. Furthermore, the mined knowledge can
be automatically updated periodically to ensure the up-to-date
view of the technology landscape.
We make the following contributions in this paper:
?We present an approach to aggregating and visualizing
the crowdsourced knowledge of technologies from Stack
Overflow to assist technology landscape inquiries;
?We implement and release the TechLand system prototype
for public use;
?We report our field deployment and two empirical studies
to evaluate the design and usefulness of the TechLand
system.

Our system have functions of complex query understanding and inference, explainable direct answer searching algorithm, similar object recommendation,
The algorithm and basic framework can also be used to search engine ranking improvement, chat robot, etc.



Finally, focusing on query understanding creates a different mindset for search engine developers. This focus shifts the emphasis from scoring and ranking to a goal of determining the searchers intent. Instead of striving to create the optimal ranking algorithm, search engine developers aspire to create the optimal query interpretation mechanism. The driving success metric is query performance ?an end-to-end measure of the quality of the communication channel between the searcher and the search engine.


==> scenario.tex <==
%\section{Motivating Scenario}
%In this session, we select a scenarios that the developers~(say Tan) may encounter when they searching online information resources, and show how our search engine assistant \emph{DeveloperBot} can assist for complex query understanding and multi-conditional querying.
%%  and exploratory search
%
%Assume that Tan is assigned a development task to extend a python-based project on a Linux operating system as shown in Fig.~\ref{queySampleFramework}.
%This project involves a large number of queries to a heterogeneous knowledge graph including RDF graphs and property graphs~\footnote[1]{https://neo4j.com/blog/rdf-triple-store-vs-labeled-property-graph-difference/}.
%Tan wants to choose the most suitable graph database for this project according to the existing environment.
%Considering upgrades and maintenance in the future, this database should satisfy the following constraints natively:
%
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=3in]{developerBot/queySampleFramework.pdf}
%    \caption {The System Framework of the Motivating Scenario}
%    \label{queySampleFramework}
%\end{figure}
%
%\begin{itemize}
%  \item This database should officially support the standard python API.
%  % and support Linux operating system
%  \item Since this database needs to store two different graph data, RDF graphs and property graphs, graph database which can be access by RDF query language will be the best choice~(instead of RDF database that only supports RDF graph).
%  \item This database needs to perform a critical operations: a large number of specific subgraph retrievals, so the RDF query language supported by this database is required to support subgraph extraction at the same time.
%\end{itemize}
%
%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=3in]{developerBot/motivatingScenario_reasoningSubgraph.pdf}
%    \caption {The Reasoning Subgraph Explanation of Direct Answer ``Virtuoso''}
%    \label{reasoningsubgraph}
%\end{figure}
%
%According to the above requirements, Tan forms the query ``Which graph databases support python and can be accessed through the RDF query languages that support subgraph extraction?'' and then input the query to the search box of \emph{DeveloperBot}.
%%then he chooses the \emph{Explainable Direct Answer} pattern and then he chooses the \emph{Explainable Direct Answer} pattern and input the query to \emph{DeveloperBot}.
%
%For this query, \emph{DeveloperBot} gives the following response:
%First, the response includes three direct answers: Amazon Neptune, Virtuoso and DB2, which are recommended graph databases that meet requirements of Tan.
%Second, each direct answer contains a reasoning subgraph to explain the reasons for recommendation.
%For example, the reasoning subgraph of the direct answer ``Virtuoso'' is shown in Fig.~\ref{reasoningsubgraph}.
%This graph explain that the direct answer ``Virtuoso''  is recommended because the ``Virtuoso'' is a graph database, and it supports Python and SPARQL.
%And the SPARQL is a RDF query language that supports subgraph extraction.
%%As shown in Fig, the confidences of Amazon Neptune, Virtuoso and DB2 are and respectively.
%Third, \emph{DeveloperBot} also gives its confidence for every direct answer.
%The above operations allow Tan to locate the three answers that meet his requirements quickly.
%%In addition, Tan can expand to see other direct answers that are not recommended but present in descending order of confidence.
%%For example, the popular graph database Neo4j is not recommended because Neo4j does not support RDF query language natively.
%
%% future work
%%But because the explanations and confidences of these answers are the same, Tan still unable to make a final decision among these three answers.
%%In this case, exploratory search providing by \emph{DeveloperBot} will help him to further understand these answers and further clarify his information needs.
%%Jimin chooses the pattern \emph{Exploratory Search} of \emph{DeveloperBot}, and input query ``Amazon Neptune, Virtuoso, DB2''.
%%As shown in Fig.??, the \emph{DeveloperBot} return two kinds of answer, called Structured Brief and Similar Object.
%%The Structured Brief provides a short textual description and a structured description for each direct answers.
%%For example, for the direct answer DB2, Structured Brief presents a short textual description like the Wikipedia and a structured description shown all the important characteristics of DB2 like all the operating systems supported by DB2, the company developed DB2, etc.
%%The Similar Object presents other objects that belong to the same category as the direct answer and the corresponding explanation.
%%Like for Amazon Neptune, Similar Object module recommends Dydra which is both a graph database and a cloud database like Amazon Neptune.
%%
%%
%%From the results of the exploratory search, Jimin learns that Amazon Neptune is a cloud database.
%%Compared with Virtuoso, DB2 supports Delphi programming language natively.
%%With the exploratory search, Jimin further explores the characteristics of these databases and compares them to reclarify his requirements: 1) he needs a local graph database nor a cloud graph database, 2) in another module of this project, the developer cooperated with him used Dephi programming language. Taking into account the future adaptability, Jimin chooses DB2 as the final option.
%% future work
%
%%exploratory search: investigating, evaluating, comparing, and synthesizing,
%
%%build a website on a Ubuntu server to collect the personal information of all the employees from Microsoft.
%%So he needs to choose a database for the data store.
%%Due to Jimin is more familiar with the Microsoft programming language, and for better compatibility and confidentiality, he prefer the database which written in Microsoft programming language.
%%
%%To search for a database which satisfy all above conditions~(database written in Microsoft programming language and can run on Ubuntu) by Bing~(A web search engine owned and operated by Microsoft), Jimin use the query keywords "database, Microsoft programming language, Ubuntu".
%%The search result return by Bing including official documentation like topic "Homepage for client programming to Microsoft SQL Server", Q\&A website like "What Programming Language Would Be Best For Ubuntu Programming?", tutorials with topic "How to install PostgreSQL (PSQL) in Ubuntu 18.04", etc.
%%Jimin reads the "How to install PostgreSQL in Ubuntu 18.04" webpage, and found that \emph{PostgreSQL} is not written in
%
%%\subsection{Specified Domain Searching}
%%e.g. postgresql developed by programming language(by can be many category, like developer, company, programming language)
%
%
%%\subsection{Complex Multi-constrain Query Reasoning and Explainable Recommendation}
%
%
%%\subsection{Exploratory Search}
%
%%\subsection{Complex Query Reasoning and }
%%Multiconditional Searching
%
%%What's currently the best choice to persist graph-like structures? Graph databases (e.g. Neo4j) or RDF triple stores (e.g. Virtuoso)?
%
%%For example, we have the following use case:
%%
%%the weakly connected graph (similar to the one of scholarly papers in a collection) with nearly 10M nodes;
%%quite rare updates;
%%critical operations: retrieving particular sub-graphs, updating nodes in a given sub-graph, re-computing link analysis measures (e.g. HITS or PageRank) after updating some nodes.
%%Providing the standard API to query the data for third party applications (a la Facebook's or Twitter's) is desired as well.
%


==> userInterface.tex <==
\section{Parallel Solution of \emph{DeveloperBot}}
